Microlocal properties of seven-dimensional lemon and apple Radon transforms with applications in Compton scattering tomography

We present a microlocal analysis of two novel Radon transforms of interest in Compton Scattering Tomography (CST), which map compactly supported $L^2$ functions to their integrals over seven-dimensional sets of apple and lemon surfaces. Specifically, we show that the apple and lemon transforms are elliptic Fourier Integral Operators (FIO), which satisfy the Bolker condition. After an analysis of the full seven-dimensional case, we focus our attention on $n$-D subsets of apple and lemon surfaces with fixed central axis, where $n<7$. Such subsets of surface integrals have applications in airport baggage and security screening. When the data dimensionality is restricted, the apple transform is shown to violate the Bolker condition, and there are artifacts which occur on apple-cylinder intersections. The lemon transform is shown to satisfy the Bolker condition, when the support of the function is restricted to the strip $\{0<z<1\}$.

==> 3.4_Sobolev.tex <==


\tc{Decide whether I can say anything about this last section.}

\tred{\subsection{Further questions}
\begin{itemize}
\item Can we derive classical Sobolev estimates for the $\mathcal{R}_j$? I mean to show that $\mathcal{R}_j$ and its inverse are bounded in some Sobolev space (we've already shown the forward operator is bounded due to Bolker). I think showing that the normal operators $\mathcal{R}_j^*\mathcal{R}$ are elliptic PDO would be sufficient to show the inverse is bounded.
\end{itemize}
}


\tc{\emph{Todd check:} Check how Bolker and Sobolev continuity work
for $\dim(Y)>\dim(X)$.  Figure out ellipticity in this case--is it
even true since you can't do my standard symbol calculation when you
pull back $(\vx,\xi)$ to a finite number of points.  How do you
calculate the symbol of the composition in this case?  Then, describe
the cutoff in between $R$
and $R^*$.
\newline If this works,  that then we can choose the cutoff it so it is elliptic for
$\vx\in B$, the unit ball. Basically, you just need to find an apple
or lemon normal to each covector in $B$.}

\noindent In the following section, we consider 3-D subsets of apple and lemon surfaces which have practical motivations in CST.
In the case of the apple transform, we discover artifacts which occur
at apple-cylinder intersections, and are thus consistent with the
results of Theorem \ref{main1}.
